Uncertainty Estimation in the Real World: A Study on Music Emotion Recognition

Any data annotation for subjective tasks shows potential variations between individuals. This is particularly true for annotations of emotional responses to musical stimuli. While older approaches to music emotion recognition systems frequently addressed this uncertainty problem through probabilistic modeling, modern systems based on neural networks tend to ignore the variability and focus only on predicting central tendencies of human subjective responses. In this work, we explore several methods for estimating not only the central tendencies of the subjective responses to a musical stimulus, but also for estimating the uncertainty associated with these responses. In particular, we investigate probabilistic loss functions and inference-time random sampling. Experimental results indicate that while the modeling of the central tendencies is achievable, modeling of the uncertainty in subjective responses proves significantly more challenging with currently available approaches even when empirical estimates of variations in the responses are available.

==> reviews.tex <==
METAREVIEW

% This paper describes how (DL-based) ML models are good at modeling means but not uncertainty.

% Three reviewers evaluated the paper and believe that it makes an insightful contribution.

That said, my cursory evaluation of the paper agrees with R2 and R3 that, while insightful, the paper's contribution is limited in terms of depth of analysis. 

There are several directions the paper can take to improve its contribution, including:
1. include different solutions (maybe some that are not based on deep learning)
2. conduct more in-depth analysis of the results (find out why these models fail)
% 3. provide suggestions for better solutions to model uncertainty (based on insights from the paper)

Aside from this, the positioning the paper can be improved in the introduction and related work sections.

Given the limited depth of the paper, I do not think it is suitable to accept it as a full paper in its current form. However, I'm willing to consider it as a "Findings" paper. If the paper gets accepted as such, the review team still suggests that the authors should add a more in-depth discussion of the possible reasons *why* these models do not perform well in this task (e.g. the models do not learn, the data is too small or sparse, the task is too difficult, etc.). 

This would be helpful for future researchers aiming to study this phenomenon in more depth and/or aiming to resolve the performance problem.


% REVIEW 1

% % ----------- Strengths -----------
% % The main strengths of the work are:

% %  - It is clear and well-written
% %  - Technically sound
% %  - Addresses an important problem

% ----------- Limitations -----------
% The main weaknesses of the work are:
%  - Additional foundational models can be used to make a stronger conclusion
%  - Other communities may be closer to the task of music emotion recognition
%  - Even if listed as future work, it would make a stronger contribution if the work proposes some alternative method to estimate the uncertainty



% ----------- Detailed comments to authors -----------

% The work studies the capacity of current approaches to estimate uncertainty in the task of music emotion recognition, which is characterized by an inherently high disagreement between annotators. 

% In this work, 5 alternative methods are compared and the results show a
% while it is possible to predict the mean it fails to estimate the uncertainty of the annotations. The work is clear, has a good structure, and is well-written. The work is technically sound and addresses an important topic.

The only point of improvement that I see is that the work only focuses on a single foundational model to base the conclusion that the proposed methods can't correctly predict the uncertainty of annotations. 

% I think to make the contribution stronger it would be better to compare multiple/different foundational models, e.g., self-supervised models or even audio features-based models.

% Finally, I think this work fits the topics of the call but it may have a larger impact in other venues such as ISMIR or ICASSP.



REVIEW 2


----------- Limitations -----------
The experiments are limited, and the contributions is not be enough for a full paper.


----------- Detailed comments to authors -----------

The paper presents an analysis of 5 deep learning methods to learn empirical distributions (mean and standard deviation). The task is Music Emotion Recognition (MER), where the ground-truth is highly subjective, therefore predicting a distribution of labels is more suitable than predicting a single label, as in standard classification tasks. Experimental results on 1 public dataset show that available models can predict mean with reasonable accuracy, but they all fail in predicting the standard deviation.

The paper is clear, easy to follow and the experimental results show a clear gap in the state-of-the-art, calling for novel methods to model uncertainty. 

However, the main contribution of the paper is an experimental comparison of the effectiveness of existing methods on a single dataset. 

While the results are interesting, the analyses and discussion are somehow limited and the reader is left with many questions. 

For example, it is unclear why the models fail in predicting uncertainty and if this behaviour has been reported in other tasks. 

An error analysis will make the paper stronger. 

Another aspect that is overlooked is efficiency. The paper mentions that some models are more efficient than others, it would be interesting to see also an efficiency comparison.


REVIEW 3


% ----------- Strengths -----------
% - Code with a readme is shared anonymously increasing the potential reproducibility of the paper.
% - Overall, the paper is clearly written and easy to follow
% - Figures are clear and help the reader in their understanding of the text.


----------- Limitations -----------
- The motivation of the task, relevance to the conference as well as choices made in the paper are lacking, which makes it difficult to understand the contribution that this paper makes to the field.

- The paper is not positioned well enough in the existing literature and it is unclear whether the approaches compared in the paper are state of the art or representative of methods used in the field of estimating aleatoric uncertainty in ML models. It seems like the chosen approaches do not all fit the task very well.

- The analysis should go more in-depth. The results are overall negative, which is not necessarily a problem in itself, but the analysis of the results as well as the discussion stays on a rather surface level, not giving much insight into reasons for why the approaches do not perform well and what could be done to improve that. This is something that would be expected from a work on comparing existing approaches on a specific task.



----------- Detailed comments to authors -----------
% - Introduction should also include a motivation for MER itself. In the current version of the paper it does not become clear why trustworthynesss and accurate uncertainty estimation is of greater importance in this particular task.

- Related work is a bit light on citations for relevant statements, especially in the "uncertainty quantification" subsection. It does not become clear why the exact methods that are compared are chosen and whether this is a complete analysis of all existing approaches (bayesian approaches are missing?) and if not why this subset of approaches was chosen.

- Related work should also position the paper more clearly in the existing literature. As an example: Are there other papers that compare different approaches to estimate aleatoric uncertainty in other tasks?

% - Typo in title of Section 2.2: Recogntion

% - Valence and arousal need to be defined in the paper. As is the reader can not follow the analysis since there are no definition of these central concepts within the paper.

% - Overall notation should be defined more carefully.  As an example: it is nowhere defined what hat theta is.

- The chosen approaches are not motivated well enough nor explained sufficiently for the reader to understand why each of them makes sense to include in this study.

% - The random seeds and mc dropout methods are usually considered approaches to estimate model uncertainty rather than aleatoric uncertainty . I do not see why the statement  "this method is based on the assumption that variations in the model optima, thus the variations in the prediction for each stimulus, translate directly to the stimulus-dependent variations." would hold. This needs to be discussed in more detail.

% - It is unclear why the authors mention the standard deviation of valence and arousal to be gaussian. This statement does not make much sense to me.

% - Information about the normalisation of valence and arousal should be before the figure where those are analysed. Also it is unclear why the values are normalised between -0.8 and 0.8 rather than -1 and 1. Choices should overall be motivated more.

% - It is not clear to me where the drop-out is applied, in the fully connected network that sits on top of the foundational model or the foundational model itself. 

% - Also assuming that the random seeds approach only varies the fcn that sits on top of the foundational model, it is not clear what effect this would have on an ensemble approach as used in this work. There should be a reference to a work that discusses a similar approach, or at least a discussion about it. Same holds for the MC dropout in case MC dropout is only applied to the FC layer.

==> sections/related.tex <==

{%\color{red}

\subsection{Uncertainty Quantification}


% In tasks that model subjective human judgments such as quality ratings, however, modeling of data uncertainty can be of crucial importance. In particular, this allows the characterization of the so-called ``ground truth'' as a distribution instead of one fixed value. 

% Few works explicitly utilizing uncertainty quantification have targeted domains adjacent to emotion recognition or audio processing. Moreover, while many works in the audio domains have utilized probabilistic modeling (see \Cref{sec:mer}), few were explicitly done to characterize uncertainties.
}

\subsection{Music Emotion Recognition} \label{sec:mer}

\edited{
Music emotion recognition (MER) is the task of predicting the emotion associated with a musical audio stimulus. MER can be formulated either as a classification task or a regression task.}
\edited{
As a classification task, MER involves associating the stimulus with one or more labels from a predefined set of emotion ``classes''. MER as a classification task is very similar to automatic music tagging and genre classification.} 
\edited{
Another formulation of MER is that of regression, with one or more numerical scales each representing a different ``dimension'' of emotion.}

\edited{
A common formation of regression-based MER involves associating a stimulus to a point in a low-dimensional ``space'' of emotion, with the most common being the valence-arousal model and variations thereof.
The V-A model is a simplified two-dimensional representation of emotion, originating from Russell's circumplex model of affect \cite{Russell1980CircumplexModelAffect}. The \textit{valence} dimension accounts for ``the degree to which an emotion is
associated with favorable outcomes'', and while the \textit{arousal} dimension accounts for ``the amount of
energy associated with an emotion''
\cite[p. 245]{Tan2018PsychologyMusicSound}. 

In this work, we will focus on the regression MER within the valence-arousal space. 

Traditional approaches to MER tend to utilize a combination of hand-designed acoustic features (e.g., MFCC, chromagram, spectral contrast) with shallow models (e.g., support vector regression) \cite{Kim2010MusicEmotionRecognition}. In 2007, Yang \etalc{}\cite{Yang2007MusicEmotionRecognition} was likely the first to address the effects of individuality on MER. Although  not directly addressing the stochasticity of subjective ratings, they  modeled emotion as a variable conditioned on the human rater. Between 2010 and 2011, Schmidt and Kim  probabilistically modeled the predicted emotion in the valence-arousal space in a series of works as a bivariate Gaussian distribution \cite{Schmidt2010PredictionTimevaryingMusical}, a bivariate Gaussian random process \cite{Schmidt2010PredictionTimeVaryingMusicala}, and a discretized distribution \cite{Schmidt2011ModelingMusicalEmotion}. 
Gaussian modeling was used again by Wang and Yang \etal{} \cite{Wang2012AcousticEmotionGaussians}, before being extended to a mixture model in \cite{Wang2015ModelingAffectiveContent, Chen2017ComponentTyingMixture}. 
Discretized grids of emotion were used by various authors in \cite{Yang2011PredictionDistributionPerceived, Wang2015HistogramDensityModeling, Chin2018PredictingProbabilityDensity}, while a random process model was further developed by Imbrasaite \etal{} in \cite{Imbrasaite2013EmotionTrackingMusic, Imbrasaite2014CCNFContinuousEmotion}. 

By the mid-2010s, deep learning approaches applied to pre-extracted acoustic features \cite{Li2016DeepBidirectionalLong, Ma2017MultiscaleContextBased, Aljanaki2017DevelopingBenchmarkEmotional} were gaining traction, particularly with the use of recurrent neural networks (RNN). In 2017, Liu~\etal{} were amongst the first to attempt a fully neural system for MER, using a convolutional neural network (CNN) on a spectrogram \cite{Liu2018AudiobasedDeepMusic}. Similar deep learning approaches continued to be used with various types of spectrograms \cite{Sarkar2020RecognitionEmotionMusic, Yang2020PredictingMusicEmotion, Hizlisoy2021MusicEmotionRecognition} and raw audio  \cite{Orjesek2019DNNBasedMusic}. Interestingly, however, none of the more contemporary neural approaches have revisited distributional modeling that was common in more traditional approaches.



% \begin{itemize}
%     \item music emotion recognition in general (maybe start with my book section as a high level summary)
%     \item problems with reliability of subjective ratings (or: maybe we do this as a section afterwards where we also show the Deam distributions etc.)
%         \begin{itemize}
%             \item should we discuss the problem with reducting a group of raters to a mean here or later or in the intro?
%         \end{itemize}
%     \item uncertainty estimation
% \end{itemize}







% \subsection{Humans are random}
% \alex{What is this here?}
% \begin{align}
%     Y \mid X, H &= f(X) + \epsilon \mid X, H + \xi \mid H\\
%     Y \mid X &= f(X) + \mathbb{E}_{H}\left\{\epsilon \mid X, H\right\} + \mathbb{E}_{H}\left\{\xi \mid H\right\}\\
%     &\coloneqq 
%     f(X) + \epsilon \mid X
% \end{align}
% $f(X)$ yields "true emotion" \yiwei{(yike)}, $f$ is a DETERMINISTIC FUNCTION, $\epsilon(X)$ is stimulus-dependent uncertainty, $\xi(H)$ is stimuli-independent uncertainty of human $H$. Assume $\mathbb{E}_H\{\xi \mid H\} = 0$ and $\mathbb{E}_{\epsilon \mid X}\{\epsilon \mid X\} = 0$

% We want to estimate 
% \begin{align}
%     \sigma^2 &= \operatorname{Var}\{Y \mid X\} = \operatorname{Var}\{\epsilon \mid X\}
% \end{align}
